Some applications of theta correspondence to branching laws

In this paper, we will use the local theta correspondences for the dual pair (Sp(W),O(V)) to investigate some branching law problems.

==> localtheta.tex <==
\section{The Local Theta Correspondences}
In this section, we will briefly recall some results about the local theta correspondence, following \cite{kudla1996notes}.
\par
Let $F$ be a local field of characteristic zero.
Consider the dual pair $\Oo(V)\times \Sp(W).$
For simplicity, we may assume that $\dim V$ is even. Fix a nontrivial additive character $\psi$ of $F.$
Let $\omega_\psi$ be the Weil representation for $\Oo(V)\times \Sp(W).$ 
%which can be describe as follows.
%Fix a Witt decomposition $W=X\oplus Y$ and let $P(Y)=GL(Y)N(Y)$ be the parabolic subgroup stabilizing the maximal isotropic subspace $Y.$ Then \[N(Y)=\{b\in Hom(X,Y)|~b^t=b \} ,\]
%where $b^t\in Hom(Y^\ast,X^\ast)\cong Hom(X,Y).$ The Weil representation $\omega_\psi$
If $\pi$ is an irreducible smooth representation of $\Oo(V)$ (\resp $\Sp(W)$), the maximal $\pi$-isotypic quotient has the form 
\[\pi\boxtimes\Theta_\psi(\pi) \]
for some smooth  representation of $\Sp(W)$ (resp. some smooth representation of $\Oo(V)$). We call $\Theta_\psi(\pi )$
the big theta lift of $\pi.$ It is known that $\Theta_\psi(\pi)$ is of finite length and hence is admissible. Let $\theta_\psi(\pi)$ be the maximal semisimple quotient of $\Theta_\psi(\pi),$ which is called the small theta lift of $\pi.$ 
\begin{theorem}[Howe duality conjecture]\cite{gan2014howe,gan2014proof}\label{localhowe}
 One has
 \begin{itemize}
 	\item $\theta_\psi(\pi)$ is irreducible whenever $\Theta_\psi(\pi)$ is non-zero.
 	\item the map $\pi\mapsto \theta_\psi(\pi)$ is injective on its domain.
 \end{itemize}
\end{theorem}
\par

 \subsection*{First Occurence Indices for pairs of orthogonal Witt Towers} Let $W_n~ (n\geq1)$ be the $2n-$dimensional symplectic vector space with associated metaplectic group $\Sp(W_n)$ and consider the two towers of orthogonal groups attached to the quadratic spaces with trivial discriminant. More precisely, let
\[V_{2r}^+= \mathbb{H}^{r}\quad\mbox{and}\quad V_{2r}^-= D\oplus\mathbb{H}^{r-2} \]
and denote the orthogonal groups by $\Oo(V_{2r}^+)$ and $\Oo(V_{2r}^-)$ respectively. For an irreducible representation $\pi$ of $\Sp(W_n),$ one may consider the theta lifts $\theta^+_{2r}(\pi)$ and $\theta^-_{2r}(\pi)$ to
$\Oo(V^+_{2r})$ and $\Oo(V_{2r}^-)$ respectively, with respect to a fixed non-trivial additive character $\psi.$ Set
\[\begin{cases}
r^+(\pi)=\inf\{2r:\theta^+_{2r}(\pi)\neq0 \};\\
r^-(\pi)=\inf\{2r:\theta^-_{2r}(\pi)\neq0 \}.
\end{cases} \]
%\begin{cases}
Then Kudla and Rallis \cite{kudla2005first}, B. Sun and C. Zhu \cite{sun2012conservation} showed:
\begin{theorem}
	[Conservation Relation] For any irreducible representation $\pi$ of $\Sp(W_n),$ we have
	\[r^+(\pi)+r^-(\pi)=4n+4=4+2\dim W_n. \]
\end{theorem}
On the other hand, one may consider the mirror situation, where one fixes an irreducible representation $\pi$ of $\Oo(V_{2r})$ and consider its theta lift $\theta_n(\pi)$ to the tower of symplectic groups $\Sp(W_n).$ Then,
with $n(\pi)$ defined in the analogous fashion
\[n(\pi)=\inf\{n:\theta_n(\pi)\neq0 \},  \]
 one has
\[n(\pi)+n(\pi\otimes\det )=2r=\dim V_{2r}. \] 

